Concept Distillation: Leveraging Human-Centered Explanations for Model Improvement

Humans use abstract concepts for understanding instead of hard features. Recent interpretability research has focused on human-centered concept explanations of neural networks. Concept Activation Vectors (CAVs) estimate a model's sensitivity and possible biases to a given concept. In this paper, we extend CAVs from post-hoc analysis to ante-hoc training in order to reduce model bias through fine-tuning using an additional Concept Loss. Concepts were defined on the final layer of the network in the past. We generalize it to intermediate layers using class prototypes. This facilitates class learning in the last convolution layer, which is known to be most informative. We also introduce Concept Distillation to create richer concepts using a pre-trained knowledgeable model as the teacher. Our method can sensitize or desensitize a model towards concepts. We show applications of concept-sensitive training to debias several classification problems. We also use concepts to induce prior knowledge into IID, a reconstruction problem. Concept-sensitive training can improve model interpretability, reduce biases, and induce prior knowledge. Please visit https://avani17101.github.io/Concept-Distilllation/ for code and more details.

==> figures/IIDconcepts.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth, height=5cm]{assets/images/IIDconcepts.pdf}
    % \vspace{-1pt}
    \caption{Concept sets used for IID experiments}
    \label{fig:IIDconepts}
\end{figure}

==> src/CAV.tex <==
\paragraph{Primer: CAV}{}
Testing with Concept Activation Vectors (TCAV) \cite{kim2018interpretability} provides model explanations via sensitvity scores of concepts. It uses directional derivatives for this. It learns a vector corresponding to a particular concept of interest and gives the model's sensitivty score towards it. For input image $x$ from the testset, layer $l$'s activation is given by $f_l(x)$. Given a concept of interest $C$, a set of images of that concept are taken as positive samples \vs a set of random images are taken as negative concept set ($C'$).
A binary linear classifier (linear regression or SVM) is used to distinguish between $l$'s activations for $C$ and $C'$ (\ie, between sets $f_l(x): x \in  C$ and $f_l(y): y \in C'$). The vector coefficient of C in the decision boundary  hyperplane is stored as the CAV, ${v}_{C}^{l}$.
Model's concept sensitivity $S_{C,l} \in [0,1]$ for a given class sample $x$ is estimated by calculating the alignment between the learned CAV $v^{l}_{C}$ and the gradient $\nabla L_{l}\left(f_{l}(\boldsymbol{x})\right)$ of loss with respect to activation for that layer (computed via back-propagation) as:
\begin{equation}
\label{eqn:grad_calc}
S_{C, l}(\boldsymbol{x}) =\nabla L_l\left(f_{l}(\boldsymbol{x})\right) \cdot \boldsymbol{v}_{C}^{l}, \quad \text{where} \quad
% where =\nabla h_{l, k}\left(f_{l}(\boldsymbol{x})\right) \cdot \boldsymbol{v}_{C}^{l}
% where  \quad 
\nabla L_{l}\left(f_{l}(\boldsymbol{x})\right) = \frac{\partial L(\boldsymbol{x})}{\partial \boldsymbol{x}_{a, b}}.
\end{equation}
TCAV has been used to analyze classifiers using a Cross-entropy (CE) loss between the predicted logit and GT class label.

Finally, the complete TCAV sensitivity score for concept $C$ is computed as the fraction of inputs ($x$'s) in the complete concept set $X$, which were positively aligned with ${v}_{C}^{l}$.
\begin{equation} \label{tcavq}
    \operatorname{TCAV}_{C,  l}=\frac{\left|\left\{\boldsymbol{x} \in X: S_{C, l}(\boldsymbol{x})< 0\right\}\right|}{\left|X\right|} 
\end{equation}

\paragraph{Primer: CDEP}{}
As mentioned before CDEP poses a loss over explanation features given as:
$$
\begin{aligned}
\hat{\theta}=\underset{\theta}{\operatorname{argmin}} & \overbrace{\sum_i \sum_c-y_{i, c} \log f_\theta\left(x_i\right)_c}^{\text {Prediction error }} \\
+\lambda & \underbrace{\sum_i \sum_S\left\|\beta\left(x_{i, S}\right)-\operatorname{expl}_{x_{i, S}}\right\|_1}_{\text {Explanation error }}
\end{aligned}
$$
% Where 
We use the above method of CDEP as a local explanation penalization term.

==> src/packages.tex <==
%% DEFAULTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{caption}
% \usepackage{subcaption}
\usepackage{multirow}

\DeclareCaptionFormat{myformat}{#3}
\captionsetup[algorithm]{format=myformat}
% \usepackage{adjustbox}

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2023} with \usepackage[nohyperref]{icml2023} above.
\usepackage{hyperref}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Use the following line for the initial blind version submitted for review:
% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2023


% ready for submission
\usepackage{neurips_2023}


% to compile a preprint version, e.g., for submission to arXiv, add add the
% [preprint] option:
%     \usepackage[preprint]{neurips_2023}
% to compile a camera-ready version, add the [final] option, e.g.:
%     \usepackage[final]{neurips_2023}
% to avoid loading the natbib package, add option nonatbib:
%    \usepackage[nonatbib]{neurips_2023}


\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{pifont}
\usepackage[symbol]{footmisc}
\renewcommand*{\thefootnote}{\fnsymbol{footnote}}


% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{algorithm}
\usepackage{algpseudocode}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}

% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
% \usepackage[textsize=tiny]{todonotes}

%% USER GIVEN %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{enumitem}
\usepackage{xspace}
\setlist{nolistsep}

% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \includegraphics[width=0.9\linewidth]


==> tables/abla.tex <==
\begin{table}[]
\begin{tabular}{ll}
\toprule
\textbf{Ablation}   & \textbf{Accuracy} \\
\midrule
% proto k=1           &                        \\
% proto k=3           &                        \\
% proto k=5           &                        \\
% proto k=7           &                        \\
% proto k=

No KDG          &      9.96                \\
Only G           &        43.               \\
L+G             &        50.93               \\
% $CAV_{loss}$        &                   \\
$CAV_{logit}$ &     25.55                 \\

% rename w/o CDEP to G
% w to L+G
\bottomrule
\end{tabular}
\caption{Our model's ablations over colormnist}
\label{tab:abla}
\end{table}
num concept sets (avg, sum)
num imgs

